A Review of Indoor Millimeter Wave Device-based Localization and Device-free Sensing Technologies and Applications

The commercial availability of low-cost millimeter wave (mmWave) communication and radar devices is starting to improve the penetration of such technologies in consumer markets, paving the way for large-scale and dense deployments in fifth-generation (5G)-and-beyond as well as 6G networks. At the same time, pervasive mmWave access will enable device localization and device-free sensing with unprecedented accuracy, especially with respect to sub-6 GHz commercial-grade devices. This paper surveys the state of the art in device-based localization and device-free sensing using mmWave communication and radar devices, with a focus on indoor deployments. We first overview key concepts about mmWave signal propagation and system design. Then, we provide a detailed account of approaches and algorithms for localization and sensing enabled by mmWaves. We consider several dimensions in our analysis, including the main objectives, techniques, and performance of each work, whether each research reached some degree of implementation, and which hardware platforms were used for this purpose. We conclude by discussing that better algorithms for consumer-grade devices, data fusion methods for dense deployments, as well as an educated application of machine learning methods are promising, relevant and timely research directions.

==> appendices_file.tex <==
\appendices

Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.




==> taxonomySummary_withCITES.tex <==
\begin{table}[h] % << PC: make it a "p" so you have it in a separate page
\caption{Summary table with citations made explicit}
\label{tab:taxSummary}

{ \centering \renewcommand{\baselinestretch}{1.0}\small 
\renewcommand{\arraystretch}{1.25}
\begin{tabular}[h!]{@{\hspace{1mm}}L{1.75cm}C{2.5cm}C{1.75cm}l C{2.5cm}C{1.5cm}C{3.5cm}@{\hspace{1mm}}}

\cmidrule[.08em]{2-7}
\multicolumn{1}{c}{\phantom{M}} & \multicolumn{6}{c}{\textbf{Indoor mmWave localization}} \\
\cmidrule{2-7}

\multicolumn{1}{c}{\phantom{M}} 
& \multicolumn{2}{c}{\textbf{Traditional methods}}
& \phantom{,}
& \multicolumn{3}{c}{\textbf{Tailored methods}} \\
\cmidrule{2-3} \cmidrule{5-7}

& \textbf{RSSI and SNR}  
& \textbf{Time information} 
& \phantom{,}
& \textbf{Angle information}
& \textbf{CSI-based}
& \textbf{Hybrid approaches} \\


\midrule

\textbf{Client-centric} 
&  \cite{5gRssi2020beam}, \cite{Vashist2020ml}, \cite{rssi2014icc}, \cite{wbfps2020Infocom}    
&    
& \phantom{,}
& \cite{olivier2016lightweight,palacios2019single}, \cite{henkAoD2020Icassp}, \cite{Yassin2017SimultaneousCI}, \cite{clam2018Palacios}, \cite{palacios2017jade} 
& 
&  \cite{BeamAoD}, \cite{polar2020Infocom},~ \cite{Yassin2018GeometricAI, MOSAIC2018slam}, \cite{3dlocmap2018Yassin}, \cite{doaLf2017}    \\ 
\midrule

\textbf{AP-centric} 
&  \cite{fing2019mitsubishi2}, \cite{deepL2020mitsubishi}, \cite{wangMERLfingerprintingPart4}  
& 
& \phantom{,}
&  \cite{Harvard2017Globecom}  
&  \cite{leap2019palacios}, \cite{tensorGSCPD}, \cite{ObjectDetAccurate2019Ajorloo}
& \cite{bielsa2018indoor}, \cite{accurate3D2018pefkianakis}, \cite{3DmmmMIMO2018Mathiopoulos}, \cite{lms2018PIMRCmotion}, \cite{losNlos2018msc}, \cite{mmRanger2019}\\
\midrule

\textbf{AP-client cooperation} 
&  \cite{fing2019mitsubishi1}
& \cite{ToF2019Maletic}
& \phantom{,}
& 
&   
& \cite{nlos2018SPAWCbrink}, \cite{pseudolateration2017},  \cite{sub6AoA2018Maletic}, \cite{kanhere2019map}\\
\bottomrule


\end{tabular}
}

\end{table}

